Preventing Representational Rank Collapse in MPNNs by Splitting the Computational Graph

The ability of message-passing neural networks (MPNNs) to fit complex functions over graphs is limited as most graph convolutions amplify the same signal across all feature channels, a phenomenon known as rank collapse, and over-smoothing as a special case. Most approaches to mitigate over-smoothing extend common message-passing schemes, e.g., the graph convolutional network, by utilizing residual connections, gating mechanisms, normalization, or regularization techniques. Our work contrarily proposes to directly tackle the cause of this issue by modifying the message-passing scheme and exchanging different types of messages using multi-relational graphs. We identify a sufficient condition to ensure linearly independent node representations. As one instantion, we show that operating on multiple directed acyclic graphs always satisfies our condition and propose to obtain these by defining a strict partial ordering of the nodes. We conduct comprehensive experiments that confirm the benefits of operating on multi-relational graphs to achieve more informative node representations.

==> sections/theory.tex <==




\section{DAGs Solve Over-Smoothing and Rank Collapse}
\label{sec:theory}
While theoretical studies on over-smoothing are available for both undirected and directed graphs, they assume ergodicity of the underlying graph, i.e.,  strongly connected and aperiodic (see ~\cref{sec:preliminaries}). This assumption is related to random walks on ergodic graphs, averaging over incoming neighbors, converging to the uniform distribution~\citep{gallager1997discrete}.
We want to investigate how removing this assumption affects message-passing and over-smoothing. A graph that is not ergodic and does not contain ergodic subgraphs is a DAG (Definition~\ref{def:dag}). We refer to nodes with no incoming edges as root nodes and nodes with no outgoing edges as leaf nodes. 
However, operating message-passing on a DAG is not immediately beneficial, as all representations converge to the zero state:
\begin{proposition} \label{prop:zero} Let $\mathbf{A}$ represent a DAG and $\mathbf{X}^{(k)}=\phi(\Tilde{\mathbf{A}}\mathbf{X}^{(k)}\mathbf{W}^{(k)})$ for any $\mathbf{W}^{(k)}\in\mathbb{R}^{d\times d^\prime}$ and a component-wise activation function $\phi$ with $\phi(0) = 0$. Then, $\lim_{l\to\infty} (\mathbf{X}^{(l)}) = \mathbf{0}\in \mathbb{R}^{n\times d}$.
\end{proposition}
\begin{proof}
    For $\mathbf{X}^{(1)}$, the representation of all root nodes is zero as they do not have any incoming messages, and $\phi(0) = 0$. As their neighbors then do not receive any non-zero messages, all states iteratively become zero.
\end{proof}

Despite all nodes ending up with the same representation, this effect differs from over-smoothing. Instead of nodes becoming more similar to each other, all signals get pushed away from the root nodes towards the leaf nodes. However, the signal is lost at the leaf nodes as they do not send any messages. Adding self-loops to all leaf nodes to maintain the signals in the graph provably prevents over-smoothing as we can state a fixed lower bound:

\begin{proposition}(DAGs do not over-smooth.)\label{prop:dag_oversmoothing}
Let $\mathbf{A}\in\mathbb{R}^{n\times n}$ represent a DAG, $\mathbf{A}_+$ the DAG with added self-loops for all leaf nodes, and $\Tilde{\mathbf{A}}_+=\mathbf{D}_+^{-1}\mathbf{A}_+$ its normalized adjacency matrix. Further let $\mathbf{X}^{(k+1)}=\Tilde{\mathbf{A}}\mathbf{X}^{(k)}\mathbf{W}^{(k)}$ for a.e. $\mathbf{W}^{(0)}\in\mathbb{R}^{d_0\times d_1},\dots,\mathbf{W}^{(k)}\in\mathbb{R}^{d_k\times d_{k+1}}$. Then, for all $l>0$ and any $\mathbf{X}^{(0)}\neq \mathbf{0}\in\mathbb{R}^{n\times d_0}$
\begin{equation*}
    E\left(\frac{\mathbf{X}^{(l)}}{||\mathbf{X}^{(l)}||_F}\right) \geq \frac{1}{n\cdot d_l}\, .
\end{equation*}
\end{proposition}
We provide the proof in Appendix~\ref{ap:math}.
Its benefit is still limited, as the representations of all non-leaf nodes become the zero vector. Similar to over-smoothing, where the smooth signal gets amplified in each iteration, here, only the signal corresponding to the particular direction gets amplified. Amplifying a single signal still leads to the more general rank collapse, which limits the performance of MPNNs~\citep{roth2023rank}.

\begin{figure*}
\definecolor{viridis1}{RGB}{72,21,103}
\definecolor{viridis2}{RGB}{40,125,142}
\definecolor{viridis3}{RGB}{115,208,85}
     \centering
     \begin{subfigure}[b]{0.21\textwidth}
         \centering
        \resizebox{\textwidth}{\textwidth}{
         \begin{tikzpicture}
\begin{scope}[every node/.style={circle,draw,scale=1.0}]
    \node (A) at (0.5,3) {};
    \node (B) at (2.5,3) {};
    \node (C) at (0,1.5) {};
    \node (D) at (1,1.5) {} ;
    \node (E) at (2,1.5) {} ;
    \node (F) at (3,1.5) {} ;
    \node (G) at (0.5,0) {} ;
    \node (H) at (1.5,0) {} ;
\end{scope}

\begin{scope}[>={Stealth[black]},
              every edge/.style={draw=black,thick}]
    \path [<->] (A) edge (B);
    \path [<->] (A) edge (C);
    \path [<->] (A) edge (E);
    \path [<->] (A) edge (G);
    \path [<->] (B) edge (D);
    \path [<->] (B) edge (E); 
    \path [<->] (B) edge (F); 
    \path [<->] (C) edge (G); 
    \path [<->] (D) edge (H); 
    \path [<->] (E) edge (H); 
    \path [<->] (C) edge (D); 
\end{scope}
\end{tikzpicture}
        }
         \caption{Original graph.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.21\textwidth}
         \centering
         \resizebox{\textwidth}{\textwidth}{
         \begin{tikzpicture}
\begin{scope}[every node/.style={circle,draw,scale=1.0}]
    \node (A) at (0.5,3) {};
    \node (B) at (2.5,3) {};
    \node (C) at (0,1.5) {};
    \node (D) at (1,1.5) {} ;
    \node (E) at (2,1.5) {} ;
    \node (F) at (3,1.5) {} ;
    \node (G) at (0.5,0) {} ;
    \node (H) at (1.5,0) {} ;
\end{scope}

\begin{scope}[>={Stealth[viridis1]},
              every edge/.style={draw=viridis1,thick}]
    \path [->] (A) edge (C);
    \path [->] (A) edge (E);
    \path [->] (A) edge (G);
    \path [->] (B) edge (D);
    \path [->] (B) edge (E); 
    \path [->] (B) edge (F); 
    \path [->] (C) edge (G); 
    \path [->] (D) edge (H); 
    \path [->] (E) edge (H); 
\end{scope}
\end{tikzpicture}
        }
         \caption{DAG.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.21\textwidth}
         \centering
         \resizebox{\textwidth}{\textwidth}{
         \begin{tikzpicture}
\begin{scope}[every node/.style={circle,draw}]
    \node (A) at (0.5,3) {};
    \node (B) at (2.5,3) {};
    \node (C) at (0,1.5) {};
    \node (D) at (1,1.5) {} ;
    \node (E) at (2,1.5) {} ;
    \node (F) at (3,1.5) {} ;
    \node (G) at (0.5,0) {} ;
    \node (H) at (1.5,0) {} ;
\end{scope}

\begin{scope}[>={Stealth[viridis2]},
              every edge/.style={draw=viridis2,thick}]
    \path [<-] (A) edge (C);
    \path [<-] (A) edge (E);
    \path [<-] (A) edge (G);
    \path [<-] (B) edge (D);
    \path [<-] (B) edge (E); 
    \path [<-] (B) edge (F); 
    \path [<-] (C) edge (G); 
    \path [<-] (D) edge (H); 
    \path [<-] (E) edge (H); 
\end{scope}
\end{tikzpicture}
        }
         \caption{Reverse DAG.}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.21\textwidth}
         \centering
         \resizebox{\textwidth}{\textwidth}{
         \begin{tikzpicture}
\begin{scope}[every node/.style={circle,draw,scale=1.0}]
    \node (A) at (0.5,3) {};
    \node (B) at (2.5,3) {};
    \node (C) at (0,1.5) {};
    \node (D) at (1,1.5) {} ;
    \node (E) at (2,1.5) {} ;
    \node (F) at (3,1.5) {} ;
    \node (G) at (0.5,0) {} ;
    \node (H) at (1.5,0) {} ;
\end{scope}

\begin{scope}[>={Stealth[viridis1]},
              every edge/.style={draw=viridis1,thick,bend right=10}]
    \path [->] (A) edge (C);
    \path [->] (A) edge (E);
    \path [->] (A) edge (G);
    \path [->] (B) edge (D);
    \path [->] (B) edge (E); 
    \path [->] (B) edge (F); 
    \path [->] (C) edge (G); 
    \path [->] (D) edge (H); 
    \path [->] (E) edge (H); 
\end{scope}
\begin{scope}[>={Stealth[viridis2]},
              every edge/.style={draw=viridis2,thick,bend left=10}]
    \path [<-] (A) edge (C);
    \path [<-] (A) edge (E);
    \path [<-] (A) edge (G);
    \path [<-] (B) edge (D);
    \path [<-] (B) edge (E); 
    \path [<-] (B) edge (F); 
    \path [<-] (C) edge (G); 
    \path [<-] (D) edge (H); 
    \path [<-] (E) edge (H); 
\end{scope}
\begin{scope}[>={Stealth[viridis3]},
              every edge/.style={draw=viridis3,thick}]
    \path [<->] (A) edge (B); 
    \path [<->] (C) edge (D); 
\end{scope}
\end{tikzpicture}
        }
         \caption{DA-MPNNs.}
     \end{subfigure}
        \caption{Different computational graphs that we consider.}
        \label{fig:comp_graphs}
\end{figure*}

We exploit the property that each DAG amplifies different signals based on their particular direction. This is contrary to any two ergodic graphs, for which random walks averaging over incoming nodes amplify the same smooth signal.
Combining multiple DAGs with distinct partial orderings allows us to amplify multiple signals simultaneously. The DAG that amplifies the most different signal in the data is its reverse DAG, which we define as follows:
\begin{definition} (Reverse DAG)
    For a given DAG $\mathcal{G} = (\mathcal{V},\mathcal{E})$, its reverse DAG is defined as $\mathcal{G}^\prime = (V,\mathcal{E}^\prime)$ with $\mathcal{E}^\prime = \{(j,i) \mid (i,j) \in\mathcal{E}\}$.
\end{definition}

When operating on these two computational graphs, we amplify multiple signals in the data simultaneously as long as we use different feature transformations. This provably prevents the rank collapse of feature representations and ensures that all representations are non-zero: 

\begin{theorem}
\label{pr:rank}(Combining DAGs prevents rank collapse.)
    Let $\mathbf{A}_1\in\mathbb{R}^{n\times n}$ represent a DAG and $\mathbf{A}_2\in\mathbb{R}^{n\times n}$ represent its reverse DAG. We assume each node to have at least one incoming edge in either $\mathbf{A}_1$ or $\mathbf{A}_2$. The row-wise vector inequality is denoted as $\neq_{\textrm{rw}}$. Let $\mathbf{X}^{(k+1)} = \mathbf{A}_1\mathbf{X}^{(k)}\mathbf{W}^{(k)}_1 + \mathbf{A}_2\mathbf{X}^{(k)}\mathbf{W}^{(k)}_2$.
    %Then, any state $\mathbf{X}^{(l)}$ with $\mathrm{rank}(\mathbf{X}^{(l)}) = 1$ is not a fixed point. 
    Then, for all $l>0$ and almost every $\mathbf{W}^{(k)}_1,\mathbf{W}^{(k)}_2\in\mathbb{R}^{d_k\times d_{k+1}}$ and $\mathbf{X}^{(0)}\neq_{\textrm{rw}} \mathbf{0}\in\mathbb{R}^{n\times d_k}$ we have
    \begin{equation}
    \mathbf{X}^{(l)}\neq_{\textrm{rw}} \mathbf{0} \land \mathrm{rank}(\mathbf{X}^{(l)}) > 1\, .
    \end{equation}
\end{theorem}

The proof shows the critical importance of employing different feature transformations for each computational graph. We avoid rank collapse as long as both $\mathbf{W}^{(k)}_1$ and $\mathbf{W}^{(k)}_2$ map a vector to two linearly independent vectors, which explains that the statement holds for almost every $\mathbf{W}^{(k)}_1,\mathbf{W}^{(k)}_2$ with respect to the Lebesgue measure. This even holds in the non-linear case, as long as this property holds for the employed activation functions, e.g., Leaky ReLU or Sigmoid:

\begin{remark}
    \cref{pr:rank} holds for any activation function $\phi$ that does not map two linearly independent vectors onto linearly dependent vectors, i.e., $\forall \mathbf{x},\mathbf{y}\in\mathbb{R}^d, \forall a,b\in\mathbb{R}, \mathbf{x} \neq a\cdot\mathbf{y} \colon \phi(\mathbf{x})\neq b\cdot\phi(\mathbf{y})$.
\end{remark}

Our theory shows clear benefits of operating on DAGs as the computational graphs. This will be particularly valuable for tasks that require models that can capture complex dynamics, e.g., heterophilic graphs.
However, for most tasks, the given graph is not a DAG. Thus, we will next propose a method to convert any graph into DAGs to benefit from the computational advantages.  






